Post-hoc Selection of Pareto-Optimal Solutions in Search and Recommendation

Information Retrieval (IR) and Recommender Systems (RS) tasks are moving from computing a ranking of final results based on a single metric to multi-objective problems. Solving these problems leads to a set of Pareto-optimal solutions, known as Pareto frontier, in which no objective can be further improved without hurting the others. In principle, all the points on the Pareto frontier are potential candidates to represent the best model selected with respect to the combination of two, or more, metrics. To our knowledge, there are no well-recognized strategies to decide which point should be selected on the frontier. In this paper, we propose a novel, post-hoc, theoretically-justified technique, named "Population Distance from Utopia" (PDU), to identify and select the one-best Pareto-optimal solution from the frontier. In detail, PDU analyzes the distribution of the points by investigating how far each point is from its utopia point (the ideal performance for the objectives). The possibility of considering fine-grained utopia points allows PDU to select solutions tailored to individual user preferences, a novel feature we call "calibration". We compare PDU against existing state-of-the-art strategies through extensive experiments on tasks from both IR and RS. Experimental results show that PDU and combined with calibration notably impact the solution selection. Furthermore, the results show that the proposed framework selects a solution in a principled way, irrespective of its position on the frontier, thus overcoming the limits of other strategies.

==> old/old_derivation_with_distance.tex <==
\subsection{Derivation of NOME}
\subsubsection{Derivation with distance}
Let us take into account an objective function space $\mathbb{R}^k$, where $k$ is the number of objectives. Let us consider a dataset of $m$ samples. For each sample, we suppose to know the best possible value of each objective. Then, we can describe each sample with a $k$-dimensional vector $\mathbf{y}_i$, with $i \in \{1,\dots,m\}$, which constitutes its utopia point in the objective function space $\mathbb{R}^k$.  We denote $\mathbf{Y}=\{\mathbf{y}_i\, |\, i\in \{1,\dots,m\}\}$.

Let us work a ranking model $\mathcal{M}$ that returns $k$ objectives performance values for each sample. Similarly, as before, each sample can be represented as a $k$-dimensional vector $\mathbf{x}_i$, with $i \in \{1,\dots,m\}$, which is the model performance point for that sample in $\mathbb{R}^k$. We denote $\mathbf{X}=\{\mathbf{x}_i\, |\, i\in \{1,\dots,m\}\}$.

At this moment, each $i$-th sample is represented by $\mathbf{y}_i$ and $\mathbf{x}_i$ in the objective function space: the closer the points, the better the model $\mathcal{M}$ performs. Hence, let us define a distance function $d:\mathbb{R}^k \times \mathbb{R}^k \rightarrow \mathbb{R}$ that satisfies the conditions of non-negativity, identity, symmetry, and the triangle inequality. Then, for the $i$-th sample, the error performed by the model $\mathcal{M}$ can be described as $d(\mathbf{y}_i,\mathbf{x}_i)$. 
\fnote{La condizione di non negatività credo dovremmo toglierla! VP}

By supposing this error term is independently and identically distributed in the dataset, it has Gaussian distribution with mean $\mu=0$ and variance $\sigma^2$: $d(\mathbf{y}_i, \mathbf{x}_i) \sim \mathcal{N}(0,\sigma^2)$.
Hence, the probability density function of $d(\mathbf{y}_i,\mathbf{x}_i)$ can be written as

\begin{equation}\label{eq:pdf}
    p(d(\mathbf{y}_i,\mathbf{x}_i)) = \frac{1}{\sqrt{2\pi}\sigma}\operatorname{exp}\left(-\frac{(d(\mathbf{y}_i,\mathbf{x}_i))^2}{2\sigma^2}\right)
\end{equation}

We can note that if $\mathbf{y}_i$ and $\mathbf{x}_i$ are close, the exponent part of the equation \ref{eq:pdf} tends to $1$, and the probability increases while tending to $0$ when are far apart and the probability decreases.

Then, we compute the probability density function of the error for the entire dataset. By assuming the samples to be independent, we obtain the following expression for the likelihood function:

\begin{equation}
    %p(d(\mathbf{y}_1,\mathbf{x}_1),\dots,d(\mathbf{y}_m,\mathbf{x}_m))
    p(d(\mathbf{Y},\mathbf{X}))=\prod_{i=1}^{m}p(d(\mathbf{y}_i,\mathbf{x}_i))
\end{equation}

Since $\mathbf{y}_i$ is the (generally unattainable) output we desire to have, we are interested in finding $\mathbf{x}_i$ to maximize $p(d(\mathbf{y}_i,\mathbf{x}_i))$ for each $i\in\{i,\dots,m\}$, i.e., we desire to maximize $p(d(\mathbf{Y},\mathbf{X}))$:

\begin{equation}\label{eq:maxlikprob}
    \hat{L}=\max_{\mathbf{X}}p(d(\mathbf{Y},\mathbf{X}))
\end{equation}

Since the logarithmic function is monotone, it does not modify the maximum and minimum positions. Then, we can apply it to simply compute the likelihood function
\begin{gather}
    %p(d(\mathbf{y}_1,\mathbf{x}_1),\dots,d(\mathbf{y}_m,\mathbf{x}_m))
    \log p(d(\mathbf{Y},\mathbf{X}))=\log \prod_{i=1}^{m}p(d(\mathbf{y}_i,\mathbf{x}_i))\\
    = \sum_{i=1}^{m}\log \frac{1}{\sqrt{2\pi}\sigma}\operatorname{exp}\left(-\frac{(d(\mathbf{y}_i,\mathbf{x}_i))^2}{2\sigma^2}\right) \\
    = \sum_{i=1}^{m} \left( \log \frac{1}{\sqrt{2\pi}\sigma} + \log \operatorname{exp} \left(-\frac{(d(\mathbf{y}_i,\mathbf{x}_i))^2}{2\sigma^2} \right) \right) \\
    = m \log \frac{1}{\sqrt{2\pi}\sigma} - \sum_{i=1}^{m} \frac{(d(\mathbf{y}_i,\mathbf{x}_i))^2}{2\sigma^2} \\ \label{eq:maxlik}
    = m \log \frac{1}{\sqrt{2\pi}\sigma} - \frac{1}{2\sigma^2}\sum_{i=1}^{m} (d(\mathbf{y}_i,\mathbf{x}_i))^2  
\end{gather}
The maximization problem in Equation \ref{eq:maxlikprob} becomes:
\begin{gather}
    \hat{L}=\max_{\mathbf{X}}p(d(\mathbf{Y},\mathbf{X}))= \max_{\mathbf{X}} \log p(d(\mathbf{Y},\mathbf{X})) \\
    = \max_{\mathbf{X}} \left( m \log \frac{1}{\sqrt{2\pi}\sigma} - \frac{1}{2\sigma^2}\sum_{i=1}^{m} (d(\mathbf{y}_i,\mathbf{x}_i))^2   \right) \\ = \max_{\mathbf{X}} \left( - \frac{1}{2\sigma^2}\sum_{i=1}^{m} (d(\mathbf{y}_i,\mathbf{x}_i))^2   \right) \\ 
    = \min_{\mathbf{X}} \left(\sum_{i=1}^{m} (d(\mathbf{y}_i,\mathbf{x}_i))^2   \right)
\end{gather}
%\vincenzo{Il fattore 1/2 sigma quadro si può rimuovere?}

%\fnote{direi proprio di si! FM}

\fnote{$m log$ sparito quale termine a comune? FM}
By considering the maximization problem in Equation \ref{eq:maxlikprob},   the terms which do not contain the parameters $\mathbf{\Theta}$ can be removed since they do not modify the maximum position:
\begin{gather}
    \hat{\mathcal{L}}(\mathbf{\Theta})=\max_{\mathbf{\Theta}}p(d(\mathbf{Y},g(\mathbf{\Theta}))) =\max_{\mathbf{\Theta}}\log p(d(\mathbf{Y},g(\mathbf{\Theta}))) \\
    = \max_{\mathbf{\Theta}} \left(-\frac{1}{2} \log \left( \sum_{i=1}^m d(\mathbf{Y},g(\mathbf{\Theta})_i)^2 \right) \right) \\ = \min_{\mathbf{\Theta}} \left( \sum_{i=1}^m d(\mathbf{Y},g(\mathbf{\Theta})_i)^2 \right)
\end{gather}
where the last step is performed by observing that the logarithmic function does not change the maximum position and maximizing a function is equivalent to minimizing the negative value of that function.

\subsubsection{Similar to probabilistic interpretation of linear regression}
Let us consider the matrix $\mathbf{Y} \in \mathbb{R}^{m \times n}$ of utopia points, where $m$ is the number of samples, and $n$ is the number of features. We can approximate $\mathbf{Y}$ with a matrix $\mathbf{X} \in \mathbb{R}^{m \times n}$. In other words, we can express $\mathbf{Y} = \mathbf{X} + \mathbf{E}$, where $\mathbf{E} \in \mathbb{R}^{m \times n}$ is the column-wise distance between $\mathbf{Y}$ and $\mathbf{X}$, i.e., a certain error.

We can model the errors matrix $\mathbf{E}$ as a Multi-Variate Gaussian distribution with zero mean and covariance matrix $\Sigma$:
\begin{equation}
\begin{aligned}
    p(\mathbf{E}; 0, \Sigma) = \frac{1}{\sqrt{(2\pi)^n|\Sigma|}}e^{(-\frac{1}{2}\mathbf{E}^T\Sigma^{-1}\mathbf{E})} \\= 
    \frac{1}{\sqrt{(2\pi)^n|\Sigma|}}e^{(-\frac{1}{2}(\mathbf{Y}-\mathbf{X})^T\Sigma^{-1}(\mathbf{Y}-\mathbf{X}))}
\end{aligned}
\end{equation}


\subsubsection{KL divergence between two multivariate gaussians}
First, recall that the KL divergence between two distributions $P$ and $Q$ is defined as
\begin{equation}
    D_{K L}(P \| Q)=\mathrm{E}_P\left[\log \frac{P}{Q}\right]
\end{equation}
Also, the density function for a multivariate Gaussian (normal) distribution with mean $\mu$ and covariance matrix $\Sigma$ is
\begin{equation}
p(x)=\frac{1}{(2 \pi)^{n / 2} \operatorname{det}(\Sigma)^{1 / 2}} \exp \left(-\frac{1}{2}(x-\mu)^T \Sigma^{-1}(x-\mu)\right)
\end{equation}
Now, consider two multivariate Gaussians in $\mathbb{R}^n, P_1$ and $P_2$. We have

%\begin{equation}
%\resizebox{0.91\hsize}{!}{%
\resizebox{.95\linewidth}{!}{
 \begin{minipage}{\linewidth}
\begin{align*}
D &\left(P_1 \| P_2\right) \\
&=\mathrm{E}_{P_1}\left[\log P_1-\log P_2\right] \\
&=\frac{1}{2} \mathrm{E}_{P_1}\left[-\log \operatorname{det} \Sigma_1-\left(x-\mu_1\right)^T \Sigma_1^{-1}\left(x-\mu_1\right)+\log \operatorname{det} \Sigma_2+\left(x-\mu_2\right)^T \Sigma_2^{-1}\left(x-\mu_2\right)\right] \\
&=\frac{1}{2} \log \frac{\operatorname{det} \Sigma_2}{\operatorname{det} \Sigma_1}+\frac{1}{2} \mathrm{E}_{P_1}\left[-\left(x-\mu_1\right)^T \Sigma_1^{-1}\left(x-\mu_1\right)+\left(x-\mu_2\right)^T \Sigma_2^{-1}\left(x-\mu_2\right)\right] \\
&=\frac{1}{2} \log \frac{\operatorname{det} \Sigma_2}{\operatorname{det} \Sigma_1}+\frac{1}{2} \mathrm{E}_{P_1}\left[-\operatorname{tr}\left(\Sigma_1^{-1}\left(x-\mu_1\right)\left(x-\mu_1\right)^T\right)+\operatorname{tr}\left(\Sigma_2^{-1}\left(x-\mu_2\right)\left(x-\mu_2\right)^T\right)\right] \\
&=\frac{1}{2} \log \frac{\operatorname{det} \Sigma_2}{\operatorname{det} \Sigma_1}+\frac{1}{2} \mathrm{E}_{P_1}\left[-\operatorname{tr}\left(\Sigma_1^{-1} \Sigma_1\right)+\operatorname{tr}\left(\Sigma_2^{-1}\left(x x^T-2 x \mu_2^T+\mu_2 \mu_2^T\right)\right)\right] \\
&=\frac{1}{2} \log \frac{\operatorname{det} \Sigma_2}{\operatorname{det} \Sigma_1}-\frac{1}{2} n+\frac{1}{2} \operatorname{tr}\left(\Sigma_2^{-1}\left(\Sigma_1+\mu_1 \mu_1^T-2 \mu_2 \mu_1^T+\mu_2 \mu_2^T\right)\right) \\
&=\frac{1}{2}\left(\log \frac{\operatorname{det} \Sigma_2}{\operatorname{det} \Sigma_1}-n+\operatorname{tr}\left(\Sigma_2^{-1} \Sigma_1\right)+\operatorname{tr}\left(\mu_1^T \Sigma_2^{-1} \mu_1-2 \mu_1^T \Sigma_2^{-1} \mu_2+\mu_2^T \Sigma_2^{-1} \mu_2\right)\right) \\
&=\frac{1}{2}\left(\log \frac{\operatorname{det} \Sigma_2}{\operatorname{det} \Sigma_1}-n+\operatorname{tr}\left(\Sigma_2^{-1} \Sigma_1\right)+\left(\mu_2-\mu_1\right)^T \Sigma_2^{-1}\left(\mu_2-\mu_1\right)\right)
\end{align*}
\end{minipage}
}

==> revision_commands.tex <==
\usepackage{soul}
\usepackage{xcolor}

% available colors from the xcolor package above
%% black, blue, brown, cyan, darkgray, gray,
%% green, lightgray, lime, magenta, olive, orange,
%% pink, purple, red, teal, violet, white, yellow.

% revision commands
\newcommand{\revrm}[1]{\st{#1}}
%
\newcommand{\fm}[1]{\textcolor{orange}{#1}}
\newcommand{\fmchange}[2]{\revrm{#1}\textcolor{orange}{#2}}



==> sections/08-calibrated.tex <==
% !TEX root = ../main.tex
% !TeX spellcheck = en_US

\newpage
\appendix
\section{Popularity-Based Utopia Point}\label{app:cal}
We compute the APLT utopia value $f_2$ for each user  by using a similar approach to \textit{weighted combination of mean and standard deviation} method proposed by \citet{DBLP:journals/eswa/JugovacJL17}. We consider the set of users $\mathcal{U}$, the set of items $\mathcal{I}$, and the mean number of transaction $T$ in the training set. 

For each item $i\in\mathcal{I}$, we assess its popularity $pop_i$ by counting the number of transactions the item is involved in.  For each user $u\in\mathcal{U}$, we define the set $\Gamma_u=\{pop_i\,|\,u \text{ interacted with } i\}$. We quantify the user $u$ popularity tendencies as:
\begin{equation}
    pop_u = \alpha \cdot \mu \left(\Gamma_u\right) + \beta \cdot \sigma \left(\Gamma_u\right)
\end{equation}
where $\alpha$ and $\beta$ are set to a fixed value of 1 as done in \cite{DBLP:journals/eswa/JugovacJL17}, $\mu\left(\cdot\right)$ and $\sigma\left(\cdot\right)$ are the mean and standard deviation operators, respectively. The higher is $pop_u$, the most user $u$ has consumed mainstream items in her past interactions.

Finally, we normalize $pop_u$ and compute the APLT utopia value for each user:
\begin{equation}
    f_2^u = \frac{pop_\Psi - pop_u}{pop_\Psi - pop_\Phi}
\end{equation}
where $\Phi$ and $\Psi$ are the sets composed by $pop_i$ values such that $i$ is one of the less and most $T$ consumed items, respectively. We apply this normalization so that the higher $f_2^u$, the less popular the user profile.

==> sections/09-related.tex <==
% !TEX root = ../main.tex
% !TeX spellcheck = en_US

\section{Related Work on MOO for IR and RS}
\label{sec:related}
While a discussion of the state-of-the-art selection approaches has been provided in Section \ref{sec:baseline}, we now briefly summarize the main contributions of MOO in IR and RS. Previous works investigate the introduction of multiple criteria in IR systems, e.g., in web search and recommendation \cite{dai2011learning,10.1145/2124295.2124350,10.1145/2187836.2187894,10.1145/1963405.1963459, 10.1145/2911451.2914708,10.1145/2348283.2348385}, and product search \cite{10.1145/3077136.3080838,10.1145/2396761.2398671}. \citet{DBLP:conf/www/CarmelHLL20} propose Stochastic Label Aggregation (SLA), a technique that perform label aggregation by randomly selecting a label per training example according to a given distribution over the labels. %The authors provide a theoretical framework showing that SLA is superior to alternative aggregation approaches.
%In fact, they show that any optimal solution of the MOO generated with label aggregation can be generated by a proper parameter choice of the SLA.
In RS, \citet{DBLP:conf/recsys/LinCPSXSZOJ19} propose a scalarization based Pareto-Efficient Learning-To-Rank (PE-LTR) framework %. They learn a ranking model  by aggregating with a weighted sum the losses defined for each objective, %The novelty of the approach relies on the fact that they 
by deriving the conditions for the weighted sum weights that ensure the solution to be Pareto efficient.
In the RS area, MOO techniques are routinely exploited for optimizing multiple fairness criteria beyond relevance. \citet{DBLP:conf/wsdm/GeZYPHHZ22} propose a fairness-aware RS based on multi-objective reinforcement learning, simultaneously optimizing clickthrough rate (CTR), as a signal for relevance, and item exposure, as a signal for fairness. Moreover, \citet{wu2022multifr} employ scalarization to optimize accuracy along with both provider and consumer fairness. \citet{DBLP:conf/sigir/NaghiaeiRD22} also integrate fairness constraints from a consumer and producer-side into a %mixed-integer linear programming 
re-ranking approach. % for recommendation.
%We propose \pdu, a novel, effective \emph{post-hoc} technique for selecting one---best---Pareto-optimal solution among the ones lying in the Pareto frontier. One novel characteristic of \pdu that is very important in IR and RS is that it is the only selection technique that can be ``calibrated'', i.e., it choose the optimal solution based on ideal targets expressed on a sample level, i.e. on single queries/users.



==> sections/addforcikm.tex <==
\section{Added for CIKM}
\input{images/paretofrontscikm}

==> tables/comparison.tex <==
\begin{table*}[h!]
\caption{Overview of the \pdu and related frameworks properties. The symbol \checkmark means that the method has the specified desirability, while the symbol $-$ means that the method could not have the specified characteristic.}
\begin{tabular}{ccccccc}
\toprule
\textbf{Method} & \textbf{\begin{tabular}[c]{@{}c@{}}Suitable\\ With \textgreater 2 \\Objectives\end{tabular}} &  \textbf{\begin{tabular}[c]{@{}c@{}}Additional\\Knowledge\\Problem\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}No Need of\\ Scaling before\\ Calculation\end{tabular}} & \textbf{Deterministic} & \textbf{\begin{tabular}[c]{@{}c@{}}Equal\\Treatment of\\PF Regions\end{tabular}} & \textbf{Calibration} \\ \midrule
\textit{A-KP}             &                                 &                                        \checkmark                    & \checkmark                       &         \checkmark               &             &       \\ 
\textit{U-KP}           &             \checkmark                    &                                  \checkmark                        & $-$                    &                        &    \checkmark        &          \\ 
$\mathcal{HV}$               &       \checkmark                                                      & Reference point               & \checkmark                       &          \checkmark              &                 &     \\ 
$ED$               &                  \checkmark               &                               Utopia point                  & $-$                    &           \checkmark             &       \checkmark       &        \\ 
$WM$               &            \checkmark                     &                               Weights   Set                    & $-$                    &            \checkmark            &      \checkmark         &       \\ 
\pdu              &           \checkmark                      &                              Utopia point                  & $-$                    &          \checkmark              &        \checkmark       &    \checkmark   \\ \bottomrule
\end{tabular}
\label{tab:comparison}
\end{table*}

==> tables/easeramazon.tex <==
{\setlength{\tabcolsep}{1.0pt}
\begin{table}
\caption{Selected solutions of the \easer models trained on Amazon Music dataset in the RS scenario with \textit{Recall} and  \textit{APLT} objectives. %As for \pdu,  the utopia point values are set to 1 for both \textit{Recall} and  \textit{APLT} for each user point, while the \textit{APLT} utopia point values are computed as explained in Section~\ref{sez:expcalibrated} for C-\pdu. Concerning $\mathcal{HV}$, the reference point is set to the origin. Regarding ED, the utopia point is $\left(1, 1\right)$. Finally, the objectives are treated as equally important in WM. Note that a min\_max normalization is applied for all the methods but $\mathcal{HV}$. 
 Arrows indicate whether better stands for low $\downarrow$ or high $\uparrow$ values. The best values are in~bold.}
\label{tab:rsamazon}
 \vspace{-0.5em}
\centering
%\setlength\tabcolsep{1.4pt}
%\renewcommand{\arraystretch}{1.1}% Wider
\small
\begin{threeparttable}[para]
\rowcolors{3}{white}{gray!15}
\begin{tabular}{ccccccccc}
\toprule
            \multicolumn{ 1}{c}{\textbf{Models}} &\multicolumn{ 2}{c}{\textbf{Objectives}}&\multicolumn{6}{c}{\textbf{Selection Strategies}} \\ \midrule
              \multicolumn{ 1}{c}{$\lambda$} &   \multicolumn{ 1}{c}{Recall $\uparrow$} & \multicolumn{ 1}{c}{APLT $\uparrow$\tnote{*}} &  \multicolumn{ 1}{c}{\pdu$\downarrow$} & \multicolumn{ 1}{c}{C-\pdu$\downarrow$} &  \multicolumn{ 1}{c}{$\mathcal{HV}\uparrow$} & \multicolumn{ 1}{c}{\textit{U-KP}$\uparrow$} & \multicolumn{ 1}{c}{$ED\downarrow$} & \multicolumn{ 1}{c}{$WM\uparrow$} \\
\midrule
  0.2 &  0.0616 & 0.1982 & 10.0111 & 9.8614 &      0.1221\tnote{$\dagger$}\tnote{$\dagger$}\tnote{$\dagger$} &            81 &              1.0000 &         0.2500 \\
  0.3 &  0.0632 & 0.1976 & \textbf{10.0104}& \textbf{9.8604} &      0.1249\tnote{$\dagger$}\tnote{$\dagger$} &            79 &              0.9524 &         0.2608 \\
  0.4 &  0.0639 & 0.1966 & 10.0110 & 9.8608 &      0.1256\tnote{$\dagger$} &            74 &              0.9331 &         0.2635 \\
  0.5 &  0.0649 & 0.1952 & 10.0117 & 9.8611 &      0.1266\tnote{$\dagger$}\tnote{$\dagger$} &            70 &              0.9042 &         0.2680 \\
  0.6 &  0.0659 & 0.1944 & 10.0116 & 9.8606 &      0.1282\tnote{$\dagger$} &            57 &              0.8731 &         0.2742 \\
  0.7 &  0.0668 & 0.1931 & 10.0123 & 9.8611 &      0.1289\tnote{$\dagger$} &            58 &              0.8494 &         0.2777 \\
  0.8 &  0.0674 & 0.1921 & 10.0128 & 9.8614 &      0.1295\tnote{$\dagger$} &            48 &              0.8307 &         0.2804 \\
  0.9 &  0.0676 & 0.1908 & 10.0140 & 9.8624 &      0.1290\tnote{$\dagger$} &            66 &              0.8254 &         0.2794 \\
  1 &  0.0683 & 0.1898 & 10.0147 & 9.8628 &      \textbf{0.1295}\tnote{$\dagger$} &            49 &              0.8074 &         0.2819 \\
 10 &  0.0853 & 0.1313 & 10.0784 & 9.9160 &      0.1120\tnote{$\dagger$} &             4 &              \textbf{0.6177} &         \textbf{0.2896} \\
 20 &  0.0905 & 0.1056 & 10.1007 & 9.9351 &      0.0955\tnote{$\dagger$} &            22 &              0.7603 &         0.2757 \\
 30 &  0.0923 & 0.0934 & 10.1118 & 9.9445 &      0.0862\tnote{$\dagger$} &            34 &              0.8485 &         0.2648 \\
 40 &  0.0937 & 0.0866 & 10.1176 & 9.9495 &      0.0812\tnote{$\dagger$} &            56 &              0.8990 &         0.2616 \\
 50 &  0.0948 & 0.0822 & 10.1214 & 9.9526 &      0.0780\tnote{$\dagger$} &            73 &              0.9327 &         0.2607 \\
 60 &  0.0951 & 0.0796 & 10.1240 & 9.9548 &      0.0757\tnote{$\dagger$} &            64 &              0.9538 &         0.2572 \\
 80 &  0.0955 & 0.0766 & 10.1268 & 9.9570 &      0.0731\tnote{$\dagger$} &            \textbf{89} &              0.9780 &         0.2542 \\
120 &  0.0957 & 0.0738 & 10.1298 & 9.9595 &      0.0706\tnote{$\dagger$} &            76 &              1.0000 &         0.2500 \\
\bottomrule
\end{tabular}
\begin{tablenotes}\footnotesize
%\item[$\dagger$]$\times 10^{-4}$ 
\item[$\dagger$]$\times 10^{-1}$  
\item[*]The higher the better refers to the provider fairness point of view.
%\item[*]$\times 10^{-2}$ 
%\item[$\ddag$]$\times 10^{-5}$ 
%\item[$\mathsection$]$\times 10^{-7}$ 
\end{tablenotes}
\vspace{-1em}
\end{threeparttable}
\end{table}
}

==> tables/tree.tex <==
\begin{table*}
\caption{Selected solutions for the IR scenario. The objectives are accuracy (\textit{nDCG}), efficiency (\textit{Seconds}), and energy consumption (\textit{Joules}).  %As for \pdu,  the utopia point values are set to $\left(1,0,0\right)$ for each query point. Concerning $\mathcal{HV}$, the reference point is $\left(0.5,0.0019,0.11\right)$. Regarding ED, the utopia point is $\left(1, 0,0\right)$. Finally, the objectives are treated as equally important in WM. 
 Arrows indicate whether better stands for low $\downarrow$ or high $\uparrow$ values. The best values are in bold.} 
 \label{tab:ir}
 \vspace{-0.5em}
\centering
\setlength\tabcolsep{3pt}
\begin{threeparttable}[para]
\small
\rowcolors{7}{gray!15}{white}
\begin{tabular}{ccccccccccccccc}
\toprule
            \multicolumn{ 2}{c}{\textbf{Models}} &\multicolumn{ 3}{c}{\textbf{Objectives}}&\multicolumn{ 10}{c}{\textbf{Selection Strategies}} \\ \midrule
 \multirow{2,5}{*}{Trees}& \multirow{2,5}{*}{Leaves} & \multirow{2,5}{*}{nDCG $\uparrow$} & \multirow{2,5}{*}{Seconds $\downarrow$} & \multirow{2,5}{*}{Joules $\downarrow$} & \multicolumn{ 5}{c}{Accuracy / Efficiency} & \multicolumn{ 5}{c}{Accuracy / Efficiency / Energy}\\
\cmidrule(lr){6-10} \cmidrule(lr){11-15} 
 \multicolumn{ 2}{c}{\textbf{}}  & \multicolumn{ 3}{c}{\textbf{}} & \multicolumn{ 1}{c}{\pdu $\downarrow$} &\multicolumn{ 1}{c}{$\mathcal{HV}\uparrow$} &\multicolumn{ 1}{c}{\textit{U-KP}$\uparrow$} & \multicolumn{ 1}{c}{$ED\downarrow$} & \multicolumn{ 1}{c}{$WM\uparrow$} & \multicolumn{ 1}{c}{\pdu $\downarrow$} &\multicolumn{ 1}{c}{$\mathcal{HV}\uparrow$} &\multicolumn{ 1}{c}{$U\uparrow$} & \multicolumn{ 1}{c}{$ED\downarrow$} & \multicolumn{ 1}{c}{$WM\uparrow$}\\ \midrule % \cmidrule(lr){1-5} \cmidrule(lr){6-10} \cmidrule(lr){11-15}
 100 & 8 &  \multicolumn{1}{c}{0.5029} &  \textbf{0.34}\tnote{$\dagger$} & \textbf{0.1967}\tnote{*} & \multicolumn{1}{c}{7.5443}  &     0.5\tnote{$\ddag$}  &            76 & 0.4971 &      0.1257& 7.5443 & 5.80\tnote{$\mathsection$} & 97 &           0.4971    & 0.0835 \\
 150 & 8 &  \multicolumn{1}{c}{0.5066} &  0.45\tnote{$\dagger$} & $0.2564\tnote{*}$ & \multicolumn{1}{c}{7.5320} &     1.2\tnote{$\ddag$} &            69 &           0.4934 &      0.1267 & 7.5320  & 13.25\tnote{$\mathsection$} & 102 & 0.4934  & 0.0840\\
 300 & 8 &  \multicolumn{1}{c}{0.5116} &  0.79\tnote{$\dagger$} & $0.4597\tnote{*}$ & \multicolumn{1}{c}{7.5171} &     2.1\tnote{$\ddag$} &            82 &           0.4883 &      0.1279 & 7.5172  & 22.38\tnote{$\mathsection$} & 95 & 0.4884  & 0.0845\\
150 & 32 &  \multicolumn{1}{c}{0.5153} &  1.23\tnote{$\dagger$} & $0.7058\tnote{*}$ & \multicolumn{1}{c}{7.5043} &     2.7\tnote{$\ddag$} &            78 &           0.4847 &      0.1288 & 7.5046  & 27.99\tnote{$\mathsection$} & 98 & 0.4848  & \textbf{0.0847}\\
300 & 16 &  \multicolumn{1}{c}{0.5155} &  1.33\tnote{$\dagger$} & $0.7690\tnote{*}$ & \multicolumn{1}{c}{7.5035} &     2.7\tnote{$\ddag$} &            87 &           0.4845 &      0.1288& 7.5038  & 27.95\tnote{$\mathsection$}& \textbf{104}  & 0.4846  &  0.0846\\
200 & 32 &  \multicolumn{1}{c}{0.5158} &  1.61\tnote{$\dagger$} & $0.9297\tnote{*}$ & \multicolumn{1}{c}{7.5019} &     2.8\tnote{$\ddag$} &          94 &           0.4842 &   0.1289 & 7.5023 &  27.72\tnote{$\mathsection$} & 101 & 0.4843   & 0.0844\\
300 & 32 &  \multicolumn{1}{c}{0.5179} &  2.14\tnote{$\dagger$} & $1.2266\tnote{*}$ & \multicolumn{1}{c}{7.4953} &     \textbf{3.0}\tnote{$\ddag$} &          \textbf{106} &           0.4821 &    0.1294 & 7.4960  & \textbf{29.53}\tnote{$\mathsection$} & 90 & 0.4822  & 0.0842\\
150 & 64 &  \multicolumn{1}{c}{0.5186} &  3.21\tnote{$\dagger$} & $1.8604\tnote{*}$ & \multicolumn{1}{c}{7.4935} &     2.9\tnote{$\ddag$} &          105 &         0.4814 &    0.1296 & 7.4951  & 26.86\tnote{$\mathsection$} &  70 & 0.4817  & 0.0833\\
300 & 64 &  \multicolumn{1}{c}{0.5212} &   6.40\tnote{$\dagger$} & $3.7657\tnote{*}$ & \multicolumn{1}{c}{7.4830} &     2.7\tnote{$\ddag$} &          102 &          0.4788 &    0.1301 & \textbf{7.4904}  & 19.31\tnote{$\mathsection$} & 81 &  \textbf{0.4803}  & 0.0805\\
500 & 64 &  \multicolumn{1}{c}{0.5225}&  10.89\tnote{$\dagger$} & $6.4691\tnote{*}$   & \multicolumn{1}{c}{7.4799} &     1.8\tnote{$\ddag$} &         98 &          0.4775 &   \textbf{0.1304} & 7.4996  &   8.26\tnote{$\mathsection$} & 85 & 0.4819   & 0.0761\\
878 & 64 &  \multicolumn{1}{c}{\textbf{0.5225}} & 17.82\tnote{$\dagger$} & $10.5964\tnote{*}$ & \multicolumn{1}{c}{\textbf{7.4768}} &     0.3\tnote{$\ddag$} & 77  &         \textbf{0.4772} &    0.1303& 7.5290   &  0.19\tnote{$\mathsection$}&          103  & 0.4888  & 0.0692 \\
\bottomrule
\end{tabular}
\begin{tablenotes}\footnotesize
%\item[$\dagger$]$\times 10^{-4}$ 
\item[$\dagger$]$\times 10^{-4}$  
\item[*]$\times 10^{-2}$ 
\item[$\ddag$]$\times 10^{-5}$ 
\item[$\mathsection$]$\times 10^{-7}$ 
\end{tablenotes}
\vspace{-0.6em}
\end{threeparttable}
\end{table*}


 %\multicolumn{ 2}{c}{\pdu $\downarrow$} &\multicolumn{ 2}{c}{$\mathcal{HV}\uparrow$} &\multicolumn{ 2}{c}{$U\uparrow$} & \multicolumn{ 2}{c}{$ED\downarrow$} & \multicolumn{ 2}{c}{$WM\uparrow$}\\

==> tables/trees_backup.tex <==
\begin{table*}
\caption{Results for regression trees-based models. As for \pdu,  the utopia point values are set to 1 for $nDCG$ and to 0 for $time$ for each query point. Concerning the hypervolumes, the reference point is $\left(0.5,  9\times10^{-5}\right)$. Regarding the euclidean distance, the utopia point is $\left(1, 0\right)$. Finally, the objectives are treated as equally important in the weighted mean.}
\centering
\begin{threeparttable}[para]
\begin{tabular}{ccccccccccccccc}
\toprule
              \multicolumn{ 14}{c}{\textbf{Information Retrieval}} \\
            \midrule
            \multicolumn{ 2}{c}{\textbf{Models}} &\multicolumn{ 3}{c}{\textbf{Objectives}}&\multicolumn{ 10}{c}{\textbf{Selection Strategies}} \\ \midrule
 \multirow{2,5}{*}{Trees}& \multirow{2,5}{*}{Leaves} & \multirow{2,5}{*}{nDCG $\uparrow$} & \multirow{2,5}{*}{Second $\downarrow$} & \multirow{2,5}{*}{Joule $\downarrow$} & \multicolumn{ 2}{c}{\pdu $\downarrow$} &\multicolumn{ 2}{c}{$\mathcal{HV}\uparrow$} &\multicolumn{ 2}{c}{$U\uparrow$} & \multicolumn{ 2}{c}{$ED\downarrow$} & \multicolumn{ 2}{c}{$WM\uparrow$}\\
\cmidrule(lr){6-15} 
 \multicolumn{ 2}{c}{\textbf{}}  & \multicolumn{ 3}{c}{\textbf{}} & 2 obj.& 3 obj. & 2 obj. & 3 obj. & 2 obj.& 3 obj. & 2 obj. & 3 obj. & 2 obj. & 3 obj.\\  \midrule
 100 & 8 &  \multicolumn{1}{||c}{0.5029} &  \textbf{0.34}\tnote{$\dagger$} & \textbf{0.1967}\tnote{*} & \multicolumn{1}{||c}{7.5443} & 7.5443 &     0.5\tnote{$\ddag$} & 5.80\tnote{$\mathsection$} &            76 & 97&           0.4971 & 0.4971 &      0.1257 & 0.0835 \\
 150 & 8 &  \multicolumn{1}{||c}{0.5066} &  0.45\tnote{$\dagger$} & $0.2564\tnote{*}$ & \multicolumn{1}{||c}{7.5320} & 7.5320 &     1.2\tnote{$\ddag$} & 13.25\tnote{$\mathsection$}&            69 & 102&           0.4934 & 0.4934 &      0.1267 & 0.0840\\
 300 & 8 &  \multicolumn{1}{||c}{0.5116} &  0.79\tnote{$\dagger$} & $0.4597\tnote{*}$ & \multicolumn{1}{||c}{7.5171} & 7.5172 &     2.1\tnote{$\ddag$} & 22.38\tnote{$\mathsection$}&            82 & 95&           0.4883 & 0.4884 &      0.1279 & 0.0845\\
150 & 32 &  \multicolumn{1}{||c}{0.5153} &  1.23\tnote{$\dagger$} & $0.7058\tnote{*}$ & \multicolumn{1}{||c}{7.5043} & 7.5046 &     2.7\tnote{$\ddag$} & 27.99\tnote{$\mathsection$}&            78 & 98&           0.4847 & 0.4848 &      0.1288 & 0.0847\\
300 & 16 &  \multicolumn{1}{||c}{0.5155} &  1.33\tnote{$\dagger$} & $0.7690\tnote{*}$ & \multicolumn{1}{||c}{7.5035} & 7.5038 &     2.7\tnote{$\ddag$} & 27.95\tnote{$\mathsection$}&            87& \textbf{104} &           0.4845 & 0.4846 &      0.1288 &  0.0846\\
200 & 32 &  \multicolumn{1}{||c}{0.5158} &  1.61\tnote{$\dagger$} & $0.9297\tnote{*}$ & \multicolumn{1}{||c}{7.5019} & 7.5023 &     2.8\tnote{$\ddag$}&  27.72\tnote{$\mathsection$}&          94 & 101&           0.4842 & 0.4843  &   0.1289 & 0.0844\\
300 & 32 &  \multicolumn{1}{||c}{0.5179} &  2.14\tnote{$\dagger$} & $1.2266\tnote{*}$ & \multicolumn{1}{||c}{7.4953} & 7.4960 &     \textbf{3.0}\tnote{$\ddag$} & \textbf{29.53}\tnote{$\mathsection$}&          \textbf{106} & 90&           0.4821 & 0.4822 &    0.1294 & 0.0842\\
150 & 64 &  \multicolumn{1}{||c}{0.5186} &  3.21\tnote{$\dagger$} & $1.8604\tnote{*}$ & \multicolumn{1}{||c}{7.4935} & 7.4951 &     2.9\tnote{$\ddag$} & 26.86\tnote{$\mathsection$}&          105 &  70&         0.4814 & 0.4817 &    0.1296 & 0.0833\\
300 & 64 &  \multicolumn{1}{||c}{0.5212} &   6.40\tnote{$\dagger$} & $3.7657\tnote{*}$ & \multicolumn{1}{||c}{7.4830} & \textbf{7.4904} &     2.7\tnote{$\ddag$} & 19.31\tnote{$\mathsection$}&          102 & 81&          0.4788 &  0.4803 &    0.1301 & 0.0805\\
500 & 64 &  \multicolumn{1}{||c}{0.5225}&  10.89\tnote{$\dagger$} & $6.4691\tnote{*}$   & \multicolumn{1}{||c}{7.4799} & 7.4996 &     1.8\tnote{$\ddag$} &   8.26\tnote{$\mathsection$}&         98 & 85&          0.4775 & 0.4819  &   0.1304 & 0.0761\\
878 & 64 &  \multicolumn{1}{||c}{\textbf{0.5225}} & 17.82\tnote{$\dagger$} & $10.5964\tnote{*}$ & \multicolumn{1}{||c}{\textbf{7.4768}} & 7.5290  &     0.3\tnote{$\ddag$} &  0.19\tnote{$\mathsection$}&          103 & 77 &         0.4772 & 0.4888 &    0.1303 & 0.0692 \\
\bottomrule
\end{tabular}
\begin{tablenotes}\footnotesize
%\item[$\dagger$]$\times 10^{-4}$ 
\item[$\dagger$]$\times 10^{-4}$  
\item[*]$\times 10^{-2}$ 
\item[$\ddag$]$\times 10^{-5}$ 
\item[$\mathsection$]$\times 10^{-7}$ 
\end{tablenotes}
\end{threeparttable}
\end{table*}
%\multicolumn{ 2}{c}{\textbf{Model}} &   nDCG@10$\uparrow$ & time$\downarrow$ &  \pdu$\downarrow$ &  $\mathcal{HV}\uparrow$ & $U\uparrow$ & $ED\downarrow$ & $WM\uparrow$ \\
 %             trees & leaves & \multicolumn{ 7}{c}{}
